Robust Reinforcement Learning via Genetic Curriculum

Achieving robust performance is crucial when applying deep reinforcement learning (RL) in safety critical systems. Some of the state of the art approaches try to address the problem with adversarial agents, but these agents often require expert supervision to fine tune and prevent the adversary from becoming too challenging to the trainee agent. While other approaches involve automatically adjusting environment setups during training, they have been limited to simple environments where low-dimensional encodings can be used. Inspired by these approaches, we propose genetic curriculum, an algorithm that automatically identifies scenarios in which the agent currently fails and generates an associated curriculum to help the agent learn to solve the scenarios and acquire more robust behaviors. As a non-parametric optimizer, our approach uses a raw, non-fixed encoding of scenarios, reducing the need for expert supervision and allowing our algorithm to adapt to the changing performance of the agent. Our empirical studies show improvement in robustness over the existing state of the art algorithms, providing training curricula that result in agents being 2 - 8x times less likely to fail without sacrificing cumulative reward. We include an ablation study and share insights on why our algorithm outperforms prior approaches.

==> introduction.tex <==
\section{INTRODUCTION}

The one of the biggest challenge to applying deep reinforcement learning (RL) in safety-critical system is training a robust agent applicable across a diverse set of scenarios. Recent advances in sim2real ~\cite{akkaya2019solving, chebotar2019closing, kaushik2020fast, hansen2020self}, along with modern high-fidelity simulators, ~\cite{Dosovitskiy17, laminar2017}, makes it possible to collect realistic training data in scenarios too dangerous and difficult to do so in real life. However, even with this setup, an agent would often leave a long tail of unsolved scenarios.


In a typical RL setup, scenarios are randomly selected every time the simulator resets during a training. As an agent becomes more robust, it becomes less and less likely to collect training data in the region where the agent currently fails. Even with data, it can be difficult for an agent to learn new behaviors applicable to the rare, remaining scenarios, since the agent would often be approaching a local minima optimized towards more probable scenarios. These long tail of unsolved scenarios often acts as a bottleneck when implementing RL agents in safety critical systems.

Adversarial training is one approach towards collecting training data in the region where the protagonist does not perform well. Showing great success with classical RL ~\cite{iyengar2005robust, nilim2005robust, mannor2012lightning} and deep learning architectures ~\cite{goodfellow2014generative, kurakin2018adversarial, samangouei2018defense, xiao2018generating}, Adversarial training in RL pairs a protagonist agent with an adversary agent each playing a zero-sum game of maximizing / minimizing reward in the environment. Robust adversarial RL (RARL)~\cite{pinto2017robust} uses an adversary to apply external force to the trainee agents while risk averse robust adversarial RL (RARARL)~\cite{pan2019risk}, probabilistic action robust Markov decision process (MDP) and robust action robust MDP (PRMDP / NRMDP) ~\cite{tessler2019action} uses adversaries to inject action noise. However, such min-max set up often lead to adversary quickly converging to a worst-case scenario too difficult for the protagonist to learn. Also, some challenging situations are difficult to represent as noise, such as a particularly hard sequence of tasks or environment setup. Our approach builds upon the adversarial RL's goal of providing challenging experience by encoding scenarios lasting for several steps instead of disturbances that is calculated per step. Our approach also focuses on how scenarios can be used in conjunction that they are not only difficult but also help agent learn new skills faster.

\textcolor{red}{Fingerprint policy optimization (FPO) ~\cite{paul2018fingerprint} is one such example of defining training scenarios by encoding environment. Building upon the idea of encoding environments in classical RL ~\cite{ciosek2017offer} ~\cite{paul2018alternating}, FPO uses bayesian optimization to select training setup with the biggest performance improvement. However, these approaches have been limited to low-dimensional fixed-length encoding for training environments. We therefore will explore using non-parametric optimizers to use non-fixed length encodings, allowing our algorithm to adjust the length of encoding during training as detailed as it needs.}

Curricular learning on the other hand focuses on how training data can be ordered to improve the learning rate and performance of the converged solution. Following the concept that learning can be easier when training data is organized in a meaningful order to gradually introduce more complex concepts ~\cite{bengio2009curriculum}, curricular learning has been incorporated into various supervised learning tasks ~\cite{zaremba2014learning, bengio2015scheduled, graves2017automated, kumar2010self, jiang2015self} as well as various RL algorithms ~\cite{asada1996purposive, karpathy2012curriculum}.~\cite{held2018automatic, ivanovic2019barc, florensa2017reverse, florensa2017automatic} uses the idea of feeding a sequence of individual sub-tasks in a gradually more difficult order towards the goal task, while Self-Paced Reinforcement Learning[?] expands the idea by defining sub-tasks in a curriculum as a population of scenarios. However, as most curricular RL requires expert to define what goal tasks are, this isn't optimal in robust RL settings. In robust RL, goal is to do well across a wide variety of tasks, so sampling closer to the goal task distribution may end up sampling scenarios in which agent already knows how to solve. This paper studies dynamically defining goal tasks as scenarios the agent currently fails.

%\vspace{-0.8cm}
\begin{figure}[ht]
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{fig/POET5.jpg}}
\caption{\textcolor{red}{Curriculum generation during POET\cite{wang2019paired}. Unlike our proposed approach, POET runs training inside genetic algorithm, greatly increasing computational load}}

\label{fig:POET}
\end{center}
\vskip -0.3in
\end{figure}

Paired open-ended trailblazer (POET) ~\cite{wang2019paired} borrows several elements from genetic algorithms to automatically define what goal should be. As shown in ~\Cref{fig:POET}, POET starts by adding a pair consisting of a random agent $(A_0)$ and a random training example $(E_0)$. During an epoch, all pairs that haven't reached a satisfactory performance are trained in parallel. At the end of each epoch, a new pair is generated by adding a small random perturbation, or mutation, to an existing example and pairing it up with a new agent that inherits the parameter weights of the existing agent that performs best on the new example.  \textcolor{red}{As POET have training nested inside genetic algorithm, the algorithm is computationally expensive as resources spent by any agents not contributing to the performance of the best-performing agent is wasted. Our approach is computationally more efficient by separating running separating genetic algorithm outside of the loop. At end of each epoch, the current policy is fixed and genetic algorithm runs to generate a set of scenarios the agent cannot solve. Furthermore, POET uses mutation to generate new scenario. This makes the search for new scenario a inefficient random walk and makes it difficult to advance towards scenarios drastically different from the the starting scenario. Our approach on the other hand incorporates crossover, the processing of mixing sequences from two parents sequences to generate two offspring, to help cover a wider variety of scenarios faster.} 

\textcolor{red}{Motivated by these breakthroughs, we propose the genetic curriculum (GC) algorithm to train a robust RL agent. Using a genetic algorithm, we will at each epoch generate a training set consisting of scenarios the protagonist agent cannot currently solve. Generated by a genetic algorithm, these scenarios will be similar to each other and will act as curriculum scenarios to each other. As a non-parametric optimizer, GC will be able to use raw encoding of non-fixed length minimizing expert supervision on designing encoding method and allow curriculum to grow in complexity as the agent's performance improves.} Our empirical results show that GC outperforms several state-of-the-art RL algorithms in terms of robustness on benchmark problems. We include analysis and ablation studies providing insight on how our method achieves such performance.

%% High-level comment: I'd recommend following the outline for introductions here: https://cs.stanford.edu/people/widom/paper-writing.html
% Make sure to explain clearly what the problem. The framing of the problem should make curriculum learning seem like the inevitable solution to the problem. The detailed discussion of prior work should go in a separate related work section.

==> related_works.tex <==
\section{Related Work}

In a typical RL setup, an agent explores the state-space and dynamics by interacting with a randomly chosen environment. Initially, it struggles to make progress as many environments are too hard.  As the agent's performance improves, the problem becomes the opposite.  It wastes the bulk of its time in situations it already knows how to handle.  This does not improve its performance and the long tail of rare failure cases remains unaddressed.  One family of robust RL approaches attempts to mitigate this issue by using adversarial agents that generate training examples in which the agent cannot perform well. Ensuring robustness against uncertainty in input, dynamics, and actions, adversarial training has shown great performance in various classical RL algorithms
~\cite{iyengar2005robust} ~\cite{nilim2005robust}, ~\cite{mannor2012lightning} as well as several deep learning architectures ~\cite{goodfellow2014generative} ~\cite{kurakin2018adversarial}, ~\cite{samangouei2018defense}, ~\cite{xiao2018generating}. 

Following this approach, adversarial training for robust RL pairs a trainee agent with an adversary agent.  They play a zero-sum game each trying to maximize or minimize reward in the environment. Adversarial agents in Robust Adversarial Reinforcement Learning(RARL)~\cite{pinto2017robust} can apply external force to the trainee agents while adversarial agents in Risk Averse Robust Adversarial RL (RARARL)~\cite{pan2019risk} Probabilistic Action Robust Markov Decision Process (MDP) and Robust Action Robust MDP (PRMDP / NRMDP)~\cite{tessler2019action} perform a similar role by introducing adversarial action noise. While this zero-sum formulation sets a minimax problem where a trainee agent tries to improve its performance for worst cases, such a formulation may or may not yield increased robustness. For safety-critical systems, one is more interested in reducing the failure rate of the policy, the probability in which the agent cannot achieve the goal state within the resource constraints.  Our empirical results show that these adversarial approaches indeed are not very effective at reducing failure rates.

Rather than adversarially working against the trainee, another family of robust RL methods focuses on aiding the trainee agent to learn a desirable behavior by choosing what training example will be provided. In Off-Environment Reinforcement Learning~\cite{ciosek2017offer}, environment generation is trained alongside the trainee agent to decrease the policy gradient of the latter. ~\cite{paul2018alternating} uses Bayesian Optimization as a way of selecting training examples that would result in the biggest improvement in the trainee's performance with Fingerprint Policy Optimization (FPO) ~\cite{paul2018fingerprint} expanding the idea to deep RL. Due to the optimization methods used, these approaches have been limited to low-dimensional encodings of training environments.

Curricular learning also focuses on the effect of training examples but generates them in a set to learn a task that would be much slower if not impossible if the agent is trained directly on the goal task. Following the concept that learning can be easier when subtasks are organized in a meaningful order to gradually introduce more complex concepts ~\cite{bengio2009curriculum}, curricular learning has been incorporated into various supervised learning tasks ~\cite{zaremba2014learning} ~\cite{bengio2015scheduled} ~\cite{graves2017automated} ~\cite{kumar2010self},~\cite{jiang2015self} as well as various RL algorithms ~\cite{asada1996purposive},~\cite{karpathy2012curriculum}. With the intuition of feeding a sequence of subtasks that are easy enough for the current controller to learn and gradually moving to the goal task,  ~\cite{held2018automatic},  ~\cite{ivanovic2019barc}  ~\cite{florensa2017reverse},~\cite{florensa2017automatic} used preset rules on how an instructor can generate sub-tasks of a given goal task. These methods were mostly focused on goal tasks and sub-tasks that could be simply described with low-dimensional encodings. 

%\vspace{-0.8cm}
\begin{figure}[ht]
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{fig/POET5.png}}
\caption{Diagram of how curriculum is generated during POET[?]}
\label{fig:POET}
\end{center}
\vskip -0.3in
\end{figure}

\textcolor{blue}{Paired Open-Ended Trailblazer (POET) ~\cite{wang2019paired} mixes concepts from genetic algorithms to do automatic task identification. As shown in ~\Cref{fig:POET}, POET starts by adding a pair consisting of a random agent $(A_0)$ and a random training example $(E_0)$. At the end of each epoch, a new pair is generated by adding a small random perturbation, or mutation, to an existing example and pairing it up with a new agent that inherits the parameter weights of the existing agent that performs best on the new example. During an epoch, all pairs that haven't reached a satisfactory performance are trained in parallel. While the mutation operations ensure similarity within training examples and ease the transfer of skills, there are several limitations to using POET for robust RL training. As multiple agents are trained simultaneously, each agent only receives a fraction of the total computation and none performs as well as a single agent would if it had received all the computation.  This also leads to difficulty in finding a general policy that applies to a broad range of situations since that expertise is spread over the agents. Our proposed method differs by generating a curriculum to train one agent throughout training. Furthermore, POET's reliance on mutation alone makes curriculum search an inefficient random walk. We propose using a full genetic method with crossover and a fitness function for more efficient training.}
